Fast Algorithms for a New Relaxation of Optimal Transport

We introduce a new class of objectives for optimal transport computations of datasets in high-dimensional Euclidean spaces. The new objectives are parametrized by $\rho \geq 1$, and provide a metric space $\mathcal{R}_{\rho}(\cdot, \cdot)$ for discrete probability distributions in $\mathbb{R}^d$. As $\rho$ approaches $1$, the metric approaches the Earth Mover's distance, but for $\rho$ larger than (but close to) $1$, admits significantly faster algorithms. Namely, for distributions $\mu$ and $\nu$ supported on $n$ and $m$ vectors in $\mathbb{R}^d$ of norm at most $r$ and any $\epsilon > 0$, we give an algorithm which outputs an additive $\epsilon r$-approximation to $\mathcal{R}_{\rho}(\mu, \nu)$ in time $(n+m) \cdot \mathrm{poly}((nm)^{(\rho-1)/\rho} \cdot 2^{\rho / (\rho-1)} / \epsilon)$.

==> optimization.tex <==
% !TEX root = main.tex

\section{An Algorithm to Optimize (\ref{eq:dual})}

We now give an algorithm to optimize (\ref{eq:dual}). We will focus on the main iterative loop of the algorithm, which will maintain values of $(\alpha,\beta) \in \R^{n + m}$. The main benefit will come from the fact that total time and memory per iteration will be linear in $O(d(n+m))$, as opposed to the $O(nm)$ time and space that Sinkhorn updates takes.

We initialize the algorithm with $s = 0$ and $(\alpha, \beta) = (0,0)$. At iteration $s \geq 0$, we consider a fixed setting of $(\alpha, \beta)$, and we show how to update it to $(\alpha', \beta')$. We will always perform updates to $(\alpha, \beta)$ which remain inside the feasible region of (\ref{eq:dual}). Thus, we may assume without loss of generality that $(\alpha, \beta)$ satisfies
\begin{align}
\Ex_{\substack{\bi \sim \mu \\ \bj \sim \nu}}\left[ \left( \dfrac{(\alpha_{\bi} + \beta_{\bj})^+}{\|x_{\bi} - y_{\bj}\|_2^p}\right)^s\right] = 1. \label{eq:constraint}
\end{align}
Otherwise, the left-hand side of (\ref{eq:constraint}) must be less than $1$ (because $(\alpha,\beta)$ is feasible), and we can rescale $(\alpha,\beta)$ to satisfy (\ref{eq:constraint}) while only increasing the objective (\ref{eq:dual}).
\begin{itemize}
\item We compute the vector $\lambda = (\lambda_{\alpha} , \lambda_{\beta}) \in \R^{n + m}$ where, for $i \in [n]$ and $j \in [m]$, we have
\begin{align*}
(\lambda_{\alpha})_i &\eqdef \mu_i \Ex_{\bj \sim \nu}\left[ \dfrac{\left( (\alpha_i + \beta_{\bj})^+ \right)^{s-1}}{\|x_{i} - y_{\bj}\|_2^{ps}}\right] \qquad (\lambda_{\beta})_j \eqdef \nu_j \Ex_{\bi \sim \mu}\left[ \dfrac{\left( (\alpha_{\bi} + \beta_j)^+\right)^{s-1}}{\|x_{\bi} - y_j\|_2^{ps}}\right],
\end{align*}
and let $\tilde{\lambda} \in \R^{n+m}$ be its normalization, so $\tilde{\lambda} = \lambda / \|\lambda\|_2$.
\item Writing the vector $g = (\mu, \nu) \in \R^{n + m}$, and we consider the update direction $u = (u^{(\alpha)}, u^{(\beta)}) \in \R^{n + m}$ given by the direction $g$ orthogonal to $\tilde{\lambda}$:
\begin{align*}
u \eqdef g - \langle g, \tilde{\lambda}\rangle \cdot \tilde{\lambda}
\end{align*}
\item Finally, we consider the update in direction $u$ and re-normalize to satisfy (\ref{eq:constraint}).
\begin{align*}
(\gamma, \delta) &\leftarrow (\alpha, \beta) + \eta \cdot u \\
(\alpha', \beta') &\leftarrow \dfrac{1}{Z^{1/s}} \cdot (\gamma, \delta) \qquad\text{where}\qquad Z = \Ex_{\substack{\bi \sim \mu \\ \bj \sim \nu}}\left[ \left( \dfrac{(\gamma_{\bi} + \delta_{\bj})^+}{\|x_{\bi} - y_{\bj}\|_2^p}\right)^s\right].
\end{align*}
\end{itemize}
\paragraph{Intuition} The intuition for the above algorithm is the following. The constraint (\ref{eq:constraint}) defines a feasible convex region such that the current iterate $(\alpha,\beta)$ lies in the boundary of the region. Considering the vector $h \in \R^{n \cdot m}_{\geq 0}$ given by $h_{ij} = \left( (\alpha_i + \beta_j)^+ / \|x_i - y_j\|_2^p\right)^{s-1}$, we have:
\begin{align*}
1 = \Ex_{\substack{\bi \sim \mu \\ \bj \sim \nu}}\left[ \left( \dfrac{(\alpha_{\bi} + \beta_{\bj})^+}{\|x_{\bi} - y_{\bj}\|_2^p} \right)^s\right] = \Ex_{\substack{\bi \sim \mu \\ \bj \sim \nu}}\left[ h_{\bi\bj} \left( \dfrac{\alpha_{\bi} + \beta_{\bj}}{\|x_{\bi} - y_{\bj}\|_2^p}\right)\right] = \langle \lambda_{\alpha}, \alpha\rangle + \langle \lambda_{\beta}, \beta\rangle.
\end{align*}
Furthermore, for every feasible $(\alpha^*, \beta^*) \in \R^{n+m}$, we can use the fact that $h_{ij} \geq 0$ and H\"{o}lder's inequality to say
\begin{align*}
\langle \lambda_{\alpha}, \alpha^*\rangle + \langle \lambda_{\beta} , \beta^*\rangle &= \Ex_{\substack{\bi \sim \mu \\ \bj \sim \nu}}\left[ h_{\bi \bj} \left( \dfrac{\alpha_{\bi}^* + \beta_{\bj}^*}{\|x_{\bi} - y_{\bj}\|_2^p}\right)\right] \leq \Ex_{\substack{\bi \sim \mu \\ \bj \sim \nu}}\left[ h_{\bi \bj} \left( \dfrac{(\alpha_{\bi}^* + \beta_{\bj}^*)^+}{\|x_{\bi} - y_{\bj}\|_2^p}\right)\right]  \\
	&\leq \left(  \Ex_{\substack{\bi \sim \mu \\ \bj \sim \nu}}\left[ h_{\bi \bj}^{\rho} \right]\right)^{1/\rho} \left(  \Ex_{\substack{\bi \sim \mu \\ \bj \sim \nu}}\left[ \left( \dfrac{(\alpha_{\bi}^* + \beta_{\bj}^*)^+}{\|x_{\bi} - y_{\bj}\|_2^p}\right)^s\right]\right)^{1/s} \leq 1.
\end{align*}
In particular, the current iterate $(\alpha, \beta)$ lies on the hyperplane $H \subset \R^{n+m}$ defined by all $x \in \R^{n+m}$ where $\langle \lambda , x \rangle = 1$, and $H$ is tangent to the feasible region of (\ref{eq:dual}). Once we let $(\gamma, \delta) \leftarrow (\alpha,\beta) + \eta \cdot u$, we have
\begin{align*}
\left( \sum_{i=1}^n \mu_i \gamma_i + \sum_{j=1}^m \nu_j \delta_j\right) - \left( \sum_{i=1}^n \mu_i \alpha_i + \sum_{j=1}^n \nu_j \beta_j \right) &= \eta \langle g, u \rangle = \eta \left( \| g\|_2^2 - \langle g, \frac{\lambda}{\|\lambda\|_2}\rangle^2 \right) > 0,
\end{align*}
implying that the objective function increases. At the same time, if we let $\eta$ be small enough, then we expect $Z$ to be close enough to $1$ that the re-scaling by $Z$ will not ruin the progress we've made toward the optimum.

\paragraph{Formal Proof} To simplify the notation, we will let $x^* = (\alpha^*, \beta^*) \in \R^{n+m}$ denote the optimum of (\ref{eq:dual}), and $x = (\alpha,\beta) \in \R^{n+m}$ be the current iterate. We will set $y = (\gamma, \delta)$ and $x' = (\alpha', \beta')$. We have
\begin{align*}
\sum_{i=1}^n \mu_i( \alpha^*_i - \alpha_i) + \sum_{j=1}^m \nu_j (\beta^*_j - \beta_j) &= \langle u + \langle g, \tilde{\lambda}\rangle \tilde{\lambda}, x^* - x \rangle \leq \frac{1}{\eta} \left\langle y - x, x^* - x\right\rangle \\
		&= \frac{1}{2\eta} \left(\| x^* - x\|_2^2 - \|y - x^*\|_2^2 + \|x - y\|_2^2 \right) \\
		&= \dfrac{1}{2\eta} \left( \| x^* - x \|_2^2 - \| x' - x^*\|_2^2 \right) + \dfrac{1}{2\eta} \left( \| x' - x^*\|_2^2 - \|y - x^*\|_2^2 \right) \\
		&\qquad + \frac{\eta \| u\|_2^2}{2} ,
\end{align*}
where in the first inequality, we used the fact that $\langle \lambda, x^* \rangle \leq 1$ and $\langle \lambda, x \rangle = 1$ to say that $\langle g, \tilde{\lambda}\rangle \langle \tilde{\lambda}, x^* - x \rangle < 0$. Since $x' = y / Z$, we can re-write
\begin{align*}
\| x' - x^*\|_2^2 - \| y - x^* \|_2^2 &= \left( \|x' - x^*\|_2 - \|y - x^*\|_2 \right) \left( \|x' - x^*\|_2 + \| y - x^*\|_2 \right) \\
	&\leq \|x' - y\|_2 \left( \| x' - y \|_2 + 2 \| y - x^*\|_2\right) \leq \left| 1 - \frac{1}{Z} \right| \| y\|_2 \cdot 2 R
\end{align*}
where $R$ is an upper bound on the distance between $y$ and $x'$ to $x^*$. We now turn to upper-bound $Z$. Here, we use two facts. The first being that $(\gamma, \delta) = (\alpha, \beta) + \eta \cdot u$. Second, we will use the fact we specified $u$ so that $\langle u, \lambda \rangle = 0$. In particular, for every $i \in [n]$ and $j \in [m]$, we apply Taylor's theorem to the function $f(t) = (t^+)^s$ (which is smooth for $s > 1$), in order to write
\begin{align*}
\left( (\gamma_{i} + \delta_j)^+ \right)^s &\leq \left( (\alpha_i + \beta_j)^+ \right)^s + s\eta \left((\alpha_{i} + \beta_j)^+ \right)^{s-1} \left( u^{(\alpha)}_i + u^{(\beta)}_j\right) \\
&\qquad \qquad + \dfrac{1}{2} \cdot \eta^2\left( u^{(\alpha)}_i + u^{(\beta)}_{j}\right)^2 \cdot  \sup_t |f''(t)|,
\end{align*}
where $t\in \R$ varies over values between $(\alpha_i + \beta_j)$ and $(\gamma_i + \delta_j) = (\alpha_i + \beta_j) + \eta (u^{(\alpha)}_i + u^{(\beta)}_j)$. Since $f''(t)$ is monotonically increasing, we have that $|f''(t)| \leq s(s-1) ( (\alpha_i + \beta_j)^+)^{s-2}$ when $u_i^{(\alpha)} + u_j^{(\beta)} < 0$ and $|f''(t)| \leq s ( s-1) ( (\alpha_i + \beta_j)^+ + \eta (u_i^{(\alpha)} + u_j^{(\beta)})^+)^{s-2}$ when $u_i^{(\alpha)} + u_j^{(\beta)} > 0$. Taking both of these together, we may upper bound
\begin{align*}
\dfrac{ |f''(t)| \cdot \left( u^{(\alpha)}_i + u^{(\beta)}_j\right)^2}{2} &\leq \frac{s(s-1)}{2} \cdot \left( (\alpha_i + \beta_j)^+ \right)^{s-2} \left(  u^{(\alpha)}_i + u^{(\beta)}_j\right)^2 \\
&\qquad + \dfrac{s(s-1)}{2} \left( (\alpha_i + \beta_j)^+ + \eta(u^{(\alpha)}_i + u^{(\beta)}_j)^+ \right)^{s-2} \left( ( u^{(\alpha)}_i + u^{(\beta)}_j)^+\right)^2 \\
	&\leq s(s-1) \cdot \left( (\alpha_i + \beta_j)^+ \right)^{s-2} \left(  (u^{(\alpha)}_i)^2 + (u^{(\beta)}_j)^2 \right) \\
&\qquad + \dfrac{s(s-1)}{2} \left( (\alpha_i + \beta_j)^+ + \eta(u^{(\alpha)}_i + u^{(\beta)}_j)^+ \right)^{s-2} \left( ( u^{(\alpha)}_i + u^{(\beta)}_j)^+\right)^2,
\end{align*}
where we used the fact that $\left( u_i^{(\alpha)} + u_j^{(\beta)}\right)^2 \leq 2 u_i^{(\alpha)} + 2u_j^{(\beta)}$. We then upper-bound $Z$ by
\begin{align*}
Z &= \Ex_{\substack{\bi \sim \mu \\ \bj \sim \nu}}\left[ \left( \dfrac{(\gamma_{\bi} + \delta_{\bj})^+}{\|x_{\bi} - y_{\bj}\|_2^p}\right)^s\right] \\
&\leq \Ex_{\substack{\bi \sim \mu \\ \bj \sim \nu}}\left[ \left( \dfrac{(\alpha_{\bi} + \beta_{\bj})^+}{\|x_{\bi} - y_{\bj}\|_2^p}\right)^{s}\right] + s\eta  \Ex_{\substack{\bi \sim \mu \\ \bj \sim \nu}}\left[ \dfrac{((\alpha_{\bi} + \beta_{\bj})^+)^{s-1}}{\|x_{\bi} - y_{\bj}\|_2^{sp}} \cdot ( u^{(\alpha)}_{\bi} + u^{(\beta)}_{\bj})\right] \\
		&\qquad + \eta^2 \cdot s (s-1) \sum_{i=1}^n (u_i^{(\alpha)})^2 \left( \mu_i \Ex_{\bj \sim \nu}\left[ \dfrac{((\alpha_{i} + \beta_{\bj})^+)^{s-2}}{\|x_{i} - y_{\bj}\|_2^{ps}}\right] \right) \\
		&\qquad + \eta^2 \cdot s(s-1) \sum_{j=1}^m (u_j^{(\beta)})^2 \left(  \nu_j \Ex_{\bi \sim \mu}\left[ \dfrac{((\alpha_{\bi} + \beta_{j})^+)^{s-2}}{\|x_{\bi} - y_{j}\|_2^{ps}}\right] \right) \\
		&\qquad + \dfrac{\eta^2 \cdot s (s-1)}{2} \Ex_{\substack{\bi \sim \mu \\ \bj \sim \nu}}\left[ \dfrac{( (\alpha_{\bi} + \beta_{\bj})^+ + \eta (u_{\bi}^{(\alpha)} + u_{\bj}^{(\beta)})^+ )^{s-2} ((u_{\bi}^{(\alpha)} + u_{\bj}^{(\beta)})^+)^2}{\|x_{\bi} - y_{\bj}\|_2^{ps}}\right].
\end{align*}
Note that we have
\begin{align*}
\Ex_{\substack{\bi \sim \mu \\ \bj \sim \nu}}\left[ \left( \dfrac{(\alpha_{\bi} + \beta_{\bj})^+}{\|x_{\bi} - y_{\bj}\|_2^p}\right)^s\right] &= 1 \\
\Ex_{\substack{\bi \sim \mu \\ \bj \sim \nu}}\left[\dfrac{((\alpha_{\bi} + \beta_{\bj})^+)^{s-1}}{\|x_{\bi} - y_{\bj}\|_2^{sp}} \cdot \left(u_{\bi}^{(\alpha)} + u_{\bj}^{(\beta)}\right) \right] &= \langle u, \lambda \rangle = 0.
\end{align*}
We bound the remaining parts as follows: we may break up into the case that 
